VietMix: A Naturally-Occurring Parallel Corpus and Augmentation Framework for Vietnamese-English Code-Mixed Machine Translation

Machine translation (MT) systems universally degrade when faced with code-mixed text. This problem is more acute for low-resource languages that lack dedicated parallel corpora. This work directly addresses this gap for Vietnamese-English, a language context characterized by challenges including orthographic ambiguity and the frequent omission of diacritics in informal text. We introduce VietMix, the first expert-translated, naturally occurring parallel corpus of Vietnamese-English code-mixed text. We establish VietMix's utility by developing a data augmentation pipeline that leverages iterative fine-tuning and targeted filtering. Experiments show that models augmented with our data outperform strong back-translation baselines by up to +3.5 xCOMET points and improve zero-shot models by up to +11.9 points. Our work delivers a foundational resource for a challenging language pair and provides a validated, transferable framework for building and augmenting corpora in other low-resource settings.

==> resources/code_xinh.tex <==
% \begin{figure*}[t]
% \centering
% \begin{lstlisting}[language=Python,breaklines=true,showstringspaces=false,literate={í}{{\'i}}1]
% class CompareEnglishTranslations(dspy.Signature):
%     """You are an expert bilingual linguist in Vietnamese and English. Please choose the better English translation for the given Vietnamese source, using the provided reference translation to understand the intended meaning of the source. First, provide a rationale explaining your thought process, then
%     determine which translation is better. Output exactly one of: A, B, Tie, or BothBad"""

%     source = dspy.InputField(
%         desc="The Vietnamese source text.")
%     translation_a = dspy.InputField(
%         desc="The English translated version from model A.")
%     translation_b = dspy.InputField(
%         desc="The English translated version from model B.")
%     reference = dspy.InputField(
%         desc="A human written English reference translation.")
%     rationale = dspy.OutputField(
%         desc="A brief explanation of the thought process.")
%     better_translation: Literal['A','B','Tie','BothBad'] = dspy.OutputField(
%         desc="Which translation is better? Output exactly one of: A, B, Tie, or BothBad."
% \end{lstlisting}
% \end{figure*}
